Exploring Chain-of-Thought Reasoning for Steerable Pluralistic Alignment

Large Language Models (LLMs) are typically trained to reflect a relatively uniform set of values, which limits their applicability to tasks that require understanding of nuanced human perspectives. Recent research has underscored the importance of enabling LLMs to support steerable pluralism -- the capacity to adopt a specific perspective and align generated outputs with it. In this work, we investigate whether Chain-of-Thought (CoT) reasoning techniques can be applied to building steerable pluralistic models. We explore several methods, including CoT prompting, fine-tuning on human-authored CoT, fine-tuning on synthetic explanations, and Reinforcement Learning with Verifiable Rewards (RLVR). We evaluate these approaches using the Value Kaleidoscope and OpinionQA datasets. Among the methods studied, RLVR consistently outperforms others and demonstrates strong training sample efficiency. We further analyze the generated CoT traces with respect to faithfulness and safety.

==> majority_voting_threshold.tex <==
CGA-Wiki
\begin{tabular}{lcccc}
    \toprule
    Majority Vote Threshold &  accuracy &  precision &  recall &  f1\_score \\
    \midrule
    1 &    0.6607 &     0.6073 &  0.9095 &    0.7283 \\
    2 &    0.6905 &     0.6439 &  0.8524 &    0.7336 \\
    3 &    0.7143 &     0.6844 &  0.7952 &    0.7357 \\
    4 &    0.7119 &     0.7079 &  0.7214 &    0.7146 \\
    5 &    0.6702 &     0.7173 &  0.5619 &    0.6302 \\
    \bottomrule
\end{tabular}
Five predictions are the same 64.29\% of the times

BNC
\begin{tabular}{lcccc}
    \toprule
    Majority Vote Threshold &  accuracy &  precision &  recall &  f1\_score \\
    \midrule
    1 &    0.9016 &     0.8643 &  0.9528 &    0.9064 \\
    2 &    0.9252 &     0.9030 &  0.9528 &    0.9272 \\
    3 &    0.9382 &     0.9318 &  0.9462 &    0.9390 \\
    4 &    0.9331 &     0.9297 &  0.9370 &    0.9333 \\
    5 &    0.9134 &     0.9487 &  0.8740 &    0.9098 \\
    \bottomrule
\end{tabular}    

5 predictions are the same 89.19\% of the times

==> related_work.tex <==
\section{Related Work}
\label{sec:related-work}

